Sherlock in OSS: A Novel Approach of Content-Based Searching in Object Storage System

Object Storage Systems (OSS) inside a cloud promise scalability, durability, availability, and concurrency. However, open-source OSS does not have a specific approach to letting users and administrators search based on the data, which is contained inside the object storage, without involving the entire cloud infrastructure. Therefore, in this paper, we propose Sherlock, a novel Content-Based Searching (CoBS) architecture to extract additional information from images and documents. Here, we store the additional information in an Elasticsearch-enabled database, which helps us to search for our desired data based on its contents. This approach works in two sequential stages. First, the data will be uploaded to a classifier that will determine the data type and send it to the specific model for the data. Here, the images that are being uploaded are sent to our trained model for object detection, and the documents are sent for keyword extraction. Next, the extracted information is sent to Elasticsearch, which enables searching based on the contents. Because the precision of the models is so fundamental to the search's correctness, we train our models with comprehensive datasets (Microsoft COCO Dataset for multimedia data and SemEval2017 Dataset for document data). Furthermore, we put our designed architecture to the test with a real-world implementation of an open-source OSS called OpenStack Swift. We upload images into the dataset of our implementation in various segments to find out the efficacy of our proposed model in real-life Swift object storage.

==> algo/method-segment.tex <==
\begin{figure}
\begin{algorithmic}[1]
\Procedure{SegmentVideo}{$inP,otP,sT,eT$}
\Comment{Here, i = Input file path, o = Output file path, sT = startTime, eT = endTime}
\State $temp, fileWOExt\gets inP.rsplit()$
\State $swiftExt\gets .data$
\State $videoExt\gets .mp4$
\State $otP += join(fileWOExt.clip(swiftExt),sT,eT)$
\State $matchedFile\gets glob.glob(otP)$
\State $tStamp\gets time.time()$
\If {($mathedFile$)}
\State $pathWBF, etag \gets matchedFile.rsplit()$
\State $otP\gets join(pathWBF, etag,tStamp) + videoExt$
\State $os.rename(matchedFile[0],otP)$
\State \textbf{return  otP, etag}
\Else
\State $tempPath\gets otp + randomInt+ videoExt$
\State $clipCmnd\gets FFmpegCommand$\Comment{FFmpeg command for clipping the video segment using sT and Et \cite{ffmpeg}}
\State $output, error\gets subprocess.Popen(clipCmnd).communicate()$
\If {$output$}
\State raise Exception
\EndIf
\State $etag\gets md5(tempPath)$\Comment{New etag calculation for segment video}
\State $otP\gets join(otP,str(etag),str(tStamp)) + videoExt$
$os.rename(tempPath,otP)$
\State \textbf{return  otP, etag}
\EndIf 
\EndProcedure
\end{algorithmic}
\caption{Algorithm for segmenting video file}\label{method-segment}
\vspace*{-.2cm}
\end{figure}


==> algo/video-segmenter-algo.tex <==
\begin{figure}
\begin{algorithmic}[1]
\Procedure{VideoSegmenter}{$app,env,start\_response$}
\Comment{Each middleware has a start\_response method which need status and headers of the response}
\State $timeRange\gets env.get(Time Range Header)$
\If {$requestMethod=GET$ and $timeRange$}
\State $itr\gets app(env,start\_response)$\Comment{Here, itr is a dictionary having important attributes in OpenStack Swift, or list insatance if any error occurs}
\If {$isinstance(itr,list)$}
\State \textbf{return itr}
\EndIf \Comment{isinstance, list both are python keyword}
\State $sT,eT\gets timeRange.split()$
\State $validTimePattern\gets CheckRegex$ \Comment{Check valid time patten using Regular expressions}
\State $outF\gets SegmentedFileLocation$
\State $outputFp, etag\gets SegmentVideo(itr.\_data\_file, outF, sT, eT)$
\State $itr.\_fp\gets open(outputFp, rb)$
\State $itr.\_diskfile.\_data\_file\gets outputFp$
\State $itr.\_obj\_size\gets  os.path.getsize(output\_fp)$
\State $itr.\_etag\gets etag$
\State $UpdateHeader()$\Comment{According to new content-length and new etag of video segment}
\State $start\_response(staus[0], headers[0])$
\State \textbf{return itr}
\EndIf
\State \textbf{return app}
\EndProcedure
\end{algorithmic}
\caption{Algorithm for the VideoSegmenter middleware}\label{video-segmenter-algo}
\vspace*{-.2cm}
\end{figure}re

==> appendices.tex <==
\section{Documents for Keyword Extraction}

\subsection{Document A}

This document has been collected from the SemEval2017 Dataset \cite{Augenstein2017-lq}.
The document is as followed: 

\textit{``Deep learning (also known as deep structured learning) is part of a broader family of machine learning methods based on artificial neural networks with representation learning. Learning can be supervised, semi-supervised or unsupervised.  Deep learning architectures such as deep neural networks, deep belief networks, recurrent neural networks and convolutional neural networks have been applied to fields including computer vision, machine vision, speech recognition, natural language processing, audio recognition, social network filtering, machine translation, bioinformatics, drug design, medical image analysis, material inspection and board game programs, where they have produced results comparable to and in some cases surpassing human expert  performance.  Artificial neural networks (ANNs) were inspired by information processing and distributed communication nodes in biological systems. ANNs have various differences from biological brains. Specifically, neural networks tend to be static and sym bolic, while the biological brain of most living organisms is dynamic (plastic) and analog.  The adjective "deep" in deep learning comes from the use of multiple layers in the network. Early work showed that a linear perceptron cannot be a universal classif ier, and then that a network with a nonpolynomial activation function with one hidden layer of unbounded width can on the other hand so be. Deep learning is a modern variation which is concerned with an unbounded number of layers of bounded size, which per mits practical application and optimized implementation, while retaining theoretical universality under mild conditions. In deep learning the layers are also permitted to be heterogeneous and to deviate widely from biologically informed connectionist model s, for the sake of efficiency, trainability and understandability, whence the "structured" part.''}

\noindent

\vspace{-0.4cm}

\subsection{Document B}

This document has been collected from Aarts et al. \cite{Aarts_2013}
The document is as followed: 

\textit{``Complex Langevin (CL) dynamics  {[}1,2{]} provides an approach to circumvent the sign problem in numerical simulations of lattice field theories with a complex Boltzmann weight, since it does not rely on importance sampling. In recent years a number of stimulating results has been obtained in the context of nonzero chemical potential, in both lower and four-dimensional field theories with a severe sign problem in the thermodynamic limit  {[}3–8{]} (for two recent reviews, see e.g. Refs.  {[}9,10{]}). However, as has been known since shortly after its inception, correct results are not guaranteed  {[}11–16{]}. This calls for an improved understanding, relying on the combination of analytical and numerical insight. In the recent past, the important role played by the properties of the real and positive probability distribution in the complexified configuration space, which is effectively sampled during the Langevin process, has been clarified  {[}17,18{]}. An important conclusion was that this distribution should be sufficiently localised in order for CL to yield valid results. Importantly, this insight has recently also led to promising results in nonabelian gauge theories, with the implementation of SL(N,C) gauge cooling  {[}8,10{]}.''}

==> dummy.tex <==


% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi


The authors would like to thank...


% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to {\LaTeX}}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}

==> info9_ack.tex <==
The authors would like to thank Ruhul A. Sujon, A.S.M Ahasanul Haque, and IPV-Cloud Storage team for their help. Besides, This research was supported by IPvision Canada Inc.%\vspace*{-.3cm}

==> loadtest_1.tex <==
\begin{table*}[]
\caption{Results for TC0 before tuning}
\label{results_tc0_bf}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time} &
  \multicolumn{1}{l|}{Pre transfer} &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.019084 & 60742.78516 & 11740.33203 & 396.943604 & 123.982391 & 0.181213 & 0.020035 & 0.181265 & 0.201807 & 0.202337 \\ \hline
B & 0.028005 & 54005.11328 & 11742       & 397        & 124        & 0.199899 & 0.029095 & 0.19996  & 0.219461 & 0.220196 \\ \hline
C & 0.004699 & 43284.96484 & 11739.61816 & 396.919464 & 123.974846 & 0.241165 & 0.014015 & 0.24128  & 0.267824 & 0.274486 \\ \hline
D & 0.016236 & 50454.20703 & 11742       & 397        & 124        & 0.219792 & 0.017153 & 0.219866 & 0.239778 & 0.240297 \\ \hline
E & 0.00502  & 41436.89453 & 11739.3418  & 396.910126 & 124        & 0.253942 & 0.014245 & 0.254066 & 0.299559 & 0.306093 \\ \hline
F & 0.004529 & 43304.47266 & 11739.63477 & 396.920013 & 123.975021 & 0.24062  & 0.013669 & 0.240748 & 0.267333 & 0.27393  \\ \hline
G & 0.00554  & 44184.625   & 11742       & 397        & 124        & 0.232295 & 0.016577 & 0.232384 & 0.261546 & 0.26961  \\ \hline
H & 0.014866 & 43963.67578 & 11742       & 397        & 124        & 0.250164 & 0.015741 & 0.250259 & 0.269775 & 0.270343 \\ \hline
I & 0.00518  & 40665.79297 & 11742       & 397        & 124        & 0.25983  & 0.01497  & 0.259972 & 0.286211 & 0.292828 \\ \hline
J & 0.030641 & 59550.21094 & 11742       & 397        & 124        & 0.183136 & 0.03137  & 0.183174 & 0.200973 & 0.201464 \\ \hline
\end{tabular} 
}
\end{table*}

\begin{table*}[]
\caption{Results for TC1 before tuning}
\label{results_tc1_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.025941 & 44218.06641 & 11742       & 397        & 124        & 0.210628 & 0.026847 & 0.210681 & 0.295597 & 0.296356 \\ \hline
B & 0.028007 & 40094.87891 & 11740.78027 & 396.95874  & 124        & 0.226313 & 0.030835 & 0.226381 & 0.310806 & 0.312144 \\ \hline
C & 0.004875 & 32523.82031 & 11742       & 397        & 124        & 0.278864 & 0.016339 & 0.278988 & 0.370114 & 0.379062 \\ \hline
D & 0.02888  & 37737.80859 & 11742       & 397        & 124        & 0.257613 & 0.029798 & 0.257688 & 0.342154 & 0.342998 \\ \hline
E & 0.005202 & 31722.86719 & 11740.45703 & 396.947845 & 124        & 0.287869 & 0.015415 & 0.287953 & 0.378094 & 0.387241 \\ \hline
F & 0.004695 & 32471.86719 & 11738.99902 & 396.898529 & 123.984154 & 0.278408 & 0.015789 & 0.278544 & 0.371103 & 0.380134 \\ \hline
G & 0.005815 & 33870.49219 & 11742       & 397        & 124        & 0.259371 & 0.018575 & 0.259466 & 0.355652 & 0.366421 \\ \hline
H & 0.025132 & 33845.66406 & 11742       & 397        & 124        & 0.286241 & 0.025839 & 0.286297 & 0.372405 & 0.373271 \\ \hline
I & 0.005172 & 31428.41211 & 11742       & 397        & 124        & 0.29311  & 0.016017 & 0.293246 & 0.382293 & 0.391595 \\ \hline
J & 0.036088 & 43424.09766 & 11742       & 397        & 124        & 0.211516 & 0.036895 & 0.211562 & 0.294506 & 0.295291 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC2 before tuning}
\label{results_tc2_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.016666 & 61303.80859 & 11742 & 494.637634 & 118 & 0.192907 & 0.01802  & 0.192965 & 0.194661 & 0.195684 \\ \hline
B & 0.028009 & 56993.98438 & 11742 & 494.676666 & 118 & 0.20456  & 0.029003 & 0.204622 & 0.205325 & 0.206063 \\ \hline
C & 0.004555 & 43706.6875  & 11742 & 494.690735 & 118 & 0.252417 & 0.013446 & 0.252517 & 0.261421 & 0.269657 \\ \hline
D & 0.015336 & 51187.59766 & 11742 & 494.677704 & 118 & 0.22953  & 0.016648 & 0.229614 & 0.231076 & 0.23216  \\ \hline
E & 0.004752 & 43076.37109 & 11742 & 494.700928 & 118 & 0.25647  & 0.013766 & 0.256587 & 0.265583 & 0.27392  \\ \hline
F & 0.004524 & 44794.70703 & 11742 & 494.692596 & 118 & 0.245845 & 0.013504 & 0.24594  & 0.254876 & 0.263174 \\ \hline
G & 0.008603 & 46317.6875  & 11742 & 494.649475 & 118 & 0.237745 & 0.019059 & 0.237822 & 0.248561 & 0.258655 \\ \hline
H & 0.020079 & 44458.49219 & 11742 & 494.675659 & 118 & 0.266636 & 0.021554 & 0.266702 & 0.268365 & 0.269538 \\ \hline
I & 0.004739 & 42573.92578 & 11742 & 494.685608 & 118 & 0.259644 & 0.013798 & 0.259754 & 0.268843 & 0.27727  \\ \hline
J & 0.034873 & 60438.15234 & 11742 & 494.663757 & 118 & 0.199091 & 0.036552 & 0.19913  & 0.200547 & 0.201592 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC3 before tuning}
\label{results_tc3_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.200632 & 8288.029297 & 11742       & 495.502441 & 118        & 1.472068 & 0.491215 & 1.472116 & 1.651441 & 1.99448  \\ \hline
B & 0.028011 & 10122.91699 & 11742       & 495.457642 & 118        & 1.061443 & 0.272406 & 1.061518 & 1.246851 & 1.575193 \\ \hline
C & 0.008518 & 7939.221191 & 11742       & 495.497864 & 118        & 1.187393 & 0.27813  & 1.18751  & 1.362424 & 1.690457 \\ \hline
D & 0.19884  & 8567.459961 & 11742       & 495.483459 & 118        & 1.417034 & 0.482272 & 1.417104 & 1.59278  & 1.923229 \\ \hline
E & 0.00983  & 7846.32959  & 11742       & 495.539856 & 118        & 1.202856 & 0.278967 & 1.202953 & 1.378434 & 1.703074 \\ \hline
F & 0.008206 & 7962.175781 & 11742       & 495.48111  & 118        & 1.208611 & 0.29059  & 1.208725 & 1.385451 & 1.71428  \\ \hline
G & 0.013085 & 7755.3125   & 11729.20898 & 495        & 117.87146  & 1.199246 & 0.298278 & 1.199332 & 1.397689 & 1.728491 \\ \hline
H & 0.193529 & 7419.634277 & 11742       & 495.537689 & 118        & 1.466874 & 0.503384 & 1.466984 & 1.647716 & 1.984346 \\ \hline
I & 0.010136 & 7754.857422 & 11729.11133 & 494.972565 & 117.870476 & 1.224849 & 0.300677 & 1.224939 & 1.403824 & 1.736876 \\ \hline
J & 0.176198 & 9551.195312 & 11742       & 495.45108  & 118        & 1.327161 & 0.454495 & 1.327202 & 1.503813 & 1.840092 \\ \hline
\end{tabular} }
\end{table*}


\begin{table}[]
\caption{Results for TC6 before tuning}
\label{results_tc6_bf}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
ID &
  Lookup time &
  Download speed &
  Size Download &
  Header Size &
  Request Size &
  App conn time &
  Conn time  &
  Pre transfer  &
  Start transfer &
  Time \\ \hline
A &
  \multicolumn{1}{c|}{0.031463} &
  \multicolumn{1}{c|}{318789.0938} &
  \multicolumn{1}{c|}{11742} &
  \multicolumn{1}{c|}{397} &
  \multicolumn{1}{c|}{123.994743} &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{0.03226} &
  \multicolumn{1}{c|}{0.032261} &
  \multicolumn{1}{c|}{0.040459} &
  \multicolumn{1}{c|}{0.040518} \\ \hline
\end{tabular}
}
\end{table}


\begin{table*}[]
\caption{Results for TC7 before tuning}
\label{results_tc7_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.032118 & 528282.0625 & 11722.91602 & 396.737183 & 124        & 0        & 0.033104 & 0.033108 & 0.051514 & 0.051642 \\ \hline
B & 0.028008 & 293970.4375 & 11680.97363 & 396.159424 & 124        & 0        & 0.037151 & 0.037165 & 0.070662 & 0.071871 \\ \hline
C & 0.004442 & 365599.8438 & 11679.35352 & 396.137726 & 123.992607 & 0        & 0.023067 & 0.023118 & 0.062519 & 0.064248 \\ \hline
D & 0.040462 & 536258.5    & 11723.05273 & 396.738647 & 124        & 0        & 0.041397 & 0.041432 & 0.060239 & 0.060324 \\ \hline
E & 0.004598 & 362341.5625 & 11696.44629 & 396.374207 & 124        & 0        & 0.022558 & 0.022618 & 0.063979 & 0.065797 \\ \hline
F & 0.00447  & 364735.125  & 11677.4043  & 396.087433 & 123.992699 & 0        & 0.023572 & 0.023623 & 0.061455 & 0.063675 \\ \hline
G & 0.004902 & 328410.8438 & 11689.36426 & 396.277374 & 124        & 0        & 0.024676 & 0.024762 & 0.06443  & 0.066232 \\ \hline
H & 0.038558 & 526368.3125 & 11709.67773 & 396.556305 & 124        & 0        & 0.039501 & 0.039505 & 0.058656 & 0.058732 \\ \hline
I & 0.005307 & 42833.24219 & 11637.13574 & 395.562378 & 124        & 0.265848 & 0.032531 & 0.266014 & 0.341607 & 0.34974  \\ \hline
J & 0.054316 & 310260.4063 & 11725.13965 & 396.768005 & 124        & 0        & 0.055128 & 0.055128 & 0.076465 & 0.076535 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC8 before tuning}
\label{results_tc8_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.01634  & 793150.625  & 11742 & 496.927765 & 118        & 0 & 0.017545 & 0.017553 & 0.018657 & 0.018711 \\ \hline
B & 0.028006 & 403035.5    & 11742 & 496.922241 & 118        & 0 & 0.02901  & 0.029011 & 0.029043 & 0.029048 \\ \hline
C & 0.004241 & 542713.5625 & 11742 & 496.922028 & 118        & 0 & 0.013129 & 0.013243 & 0.021509 & 0.021669 \\ \hline
D & 0.01867  & 819641.875  & 11742 & 496.926453 & 118        & 0 & 0.019915 & 0.019918 & 0.02098  & 0.021005 \\ \hline
E & 0.004355 & 537195.6875 & 11742 & 496.904572 & 117.995857 & 0 & 0.013345 & 0.013416 & 0.021766 & 0.021968 \\ \hline
F & 0.004219 & 540506      & 11742 & 496.925079 & 118        & 0 & 0.013219 & 0.013248 & 0.021513 & 0.021775 \\ \hline
G & 0.004637 & 463077.7813 & 11742 & 496.908417 & 117.996346 & 0 & 0.01495  & 0.015119 & 0.025573 & 0.025766 \\ \hline
H & 0.016679 & 800007.125  & 11742 & 496.930511 & 118        & 0 & 0.017859 & 0.01787  & 0.01898  & 0.019023 \\ \hline
I & 0.004487 & 528053.625  & 11742 & 496.9245   & 118        & 0 & 0.013589 & 0.013639 & 0.02217  & 0.022476 \\ \hline
J & 0.031539 & 388759.25   & 11742 & 496.905762 & 117.996407 & 0 & 0.032659 & 0.032662 & 0.033766 & 0.033794 \\ \hline
\end{tabular} }
\caption{Results for TC8}
\label{results_tc8}
\end{table*}

\begin{table*}[]
\caption{Results for TC9 before tuning}
\label{results_tc9_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.035501 & 779714.875  & 11742       & 500.507355 & 118        & 0 & 0.03955  & 0.03956  & 0.041618 & 0.042822 \\ \hline
B & 0.031233 & 365632.7813 & 11742       & 500.304138 & 118        & 0 & 0.035398 & 0.035413 & 0.03876  & 0.044857 \\ \hline
C & 0.005066 & 483237.6875 & 11742       & 500.31015  & 118        & 0 & 0.019073 & 0.019181 & 0.030652 & 0.036963 \\ \hline
D & 0.04306  & 797047.0625 & 11740.50391 & 500.432404 & 117.994987 & 0 & 0.047339 & 0.047343 & 0.050148 & 0.051527 \\ \hline
E & 0.005443 & 479925.0938 & 11741.48828 & 500.289429 & 117.994858 & 0 & 0.018925 & 0.019012 & 0.030551 & 0.036844 \\ \hline
F & 0.004677 & 482887.625  & 11742       & 500.315552 & 118        & 0 & 0.01913  & 0.019178 & 0.03065  & 0.036974 \\ \hline
G & 0.004998 & 417355.4688 & 11742       & 500.327332 & 118        & 0 & 0.019258 & 0.019437 & 0.032841 & 0.038926 \\ \hline
H & 0.04442  & 783647.875  & 11741.48731 & 500.490753 & 118        & 0 & 0.048976 & 0.048988 & 0.051447 & 0.052671 \\ \hline
I & 0.00532  & 474259.5938 & 11742       & 500.314331 & 118        & 0 & 0.019547 & 0.019606 & 0.031274 & 0.037624 \\ \hline
J & 0.057037 & 380339      & 11740.93359 & 500.431732 & 117.994637 & 0 & 0.062501 & 0.062507 & 0.065914 & 0.067976 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC10 before tuning}
\label{results_tc10_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.015693 & 791184      & 11742       & 500.959412 & 118        & 0 & 0.017008 & 0.017017 & 0.018218 & 0.018355 \\ \hline
B & 0.028436 & 401120.625  & 11742       & 500.940765 & 117.995392 & 0 & 0.029506 & 0.029508 & 0.029616 & 0.029686 \\ \hline
C & 0.004224 & 540269.9375 & 11742       & 500.960327 & 118        & 0 & 0.013374 & 0.013499 & 0.021853 & 0.022126 \\ \hline
D & 0.015018 & 812451.875  & 11742       & 500.960327 & 118        & 0 & 0.016396 & 0.0164   & 0.017575 & 0.017709 \\ \hline
E & 0.004389 & 532594.25   & 11741.51563 & 500.941376 & 117.995132 & 0 & 0.013691 & 0.013759 & 0.022222 & 0.022571 \\ \hline
F & 0.004252 & 536894.25   & 11742       & 500.959534 & 118        & 0 & 0.013624 & 0.013664 & 0.022023 & 0.022366 \\ \hline
G & 0.004508 & 462244.4063 & 11742       & 500.962097 & 118        & 0 & 0.015063 & 0.01522  & 0.025754 & 0.026082 \\ \hline
H & 0.01524  & 793786.25   & 11742       & 500.962372 & 117.996124 & 0 & 0.016703 & 0.016716 & 0.017917 & 0.018047 \\ \hline
I & 0.004396 & 529712.6875 & 11742       & 500.959564 & 118        & 0 & 0.013796 & 0.01384  & 0.022363 & 0.022779 \\ \hline
J & 0.030542 & 386226.125  & 11742       & 500.959564 & 118        & 0 & 0.031954 & 0.031958 & 0.033186 & 0.033347 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC11 before tuning}
\label{results_tc11_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.019634 & 721993.6875 & 11742       & 500.908142 & 118        & 0 & 0.025823 & 0.025838 & 0.031075 & 0.039147 \\ \hline
B & 0.029113 & 354770.1563 & 11741.40918 & 500.874695 & 117.994064 & 0 & 0.03693  & 0.036943 & 0.043712 & 0.056926 \\ \hline
C & 0.004572 & 474768.75   & 11742       & 500.901184 & 118        & 0 & 0.021725 & 0.021837 & 0.036444 & 0.049059 \\ \hline
D & 0.022678 & 725800.625  & 11742       & 500.906921 & 118        & 0 & 0.030354 & 0.030365 & 0.036878 & 0.047431 \\ \hline
E & 0.005447 & 471577.6563 & 11742       & 500.874115 & 117.993446 & 0 & 0.02177  & 0.021853 & 0.036596 & 0.049283 \\ \hline
F & 0.004729 & 474586.25   & 11742       & 500.90155  & 118        & 0 & 0.021748 & 0.0218   & 0.03631  & 0.048698 \\ \hline
G & 0.004847 & 415515.6875 & 11742       & 500.900909 & 118        & 0 & 0.021476 & 0.021635 & 0.037804 & 0.049496 \\ \hline
H & 0.023517 & 718484.625  & 11742       & 500.899933 & 118        & 0 & 0.03138  & 0.0314   & 0.037769 & 0.048055 \\ \hline
I & 0.006019 & 466451.1875 & 11741.3457  & 500.874023 & 117.993423 & 0 & 0.022209 & 0.02227  & 0.037181 & 0.050129 \\ \hline
J & 0.03905  & 349520.0313 & 11742       & 500.900757 & 118        & 0 & 0.047338 & 0.047348 & 0.05411  & 0.06533  \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC12 before tuning}
\label{results_tc12_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.015487 & 65150.70313 & 11742       & 397        & 124        & 0.165426 & 0.016397 & 0.165461 & 0.182837 & 0.183459 \\ \hline
B & 0.028004 & 54259.375   & 11742       & 397        & 124        & 0.199812 & 0.029462 & 0.199873 & 0.217369 & 0.218188 \\ \hline
C & 0.004641 & 44056.16016 & 11740.15234 & 396.937531 & 123.980484 & 0.237686 & 0.014099 & 0.23782  & 0.263421 & 0.26915  \\ \hline
D & 0.015714 & 48451.64453 & 11742       & 397        & 124        & 0.228081 & 0.016631 & 0.228154 & 0.245271 & 0.245894 \\ \hline
E & 0.004814 & 43232.64063 & 11742       & 397        & 124        & 0.243494 & 0.014178 & 0.243625 & 0.268547 & 0.274406 \\ \hline
F & 0.004703 & 44301.62109 & 11740.16699 & 396.938019 & 123.980644 & 0.235781 & 0.014175 & 0.235909 & 0.2616   & 0.267554 \\ \hline
G & 0.005404 & 47149.33984 & 11740.2832  & 396.941956 & 123.981873 & 0.220683 & 0.01673  & 0.220772 & 0.248511 & 0.255698 \\ \hline
H & 0.01869  & 47133.57422 & 11742       & 397        & 124        & 0.23321  & 0.019336 & 0.233289 & 0.25055  & 0.251207 \\ \hline
I & 0.004654 & 43755.59766 & 11742       & 397        & 124        & 0.239956 & 0.01418  & 0.240084 & 0.265467 & 0.271249 \\ \hline
J & 0.029555 & 60144.29297 & 11742       & 397        & 124        & 0.180714 & 0.030234 & 0.180757 & 0.197452 & 0.198023 \\ \hline
\end{tabular} }
\caption{Results for TC12}
\label{results_tc12}
\end{table*}

\begin{table*}[]
\caption{Results for TC13 before tuning}
\label{results_tc13_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.041417 & 19062.94531 & 7828        & 264.666656 & 82.666664 & 2.036389 & 3.376111 & 2.036472 & 2.130972 & 49.295055 \\ \hline
B & 0.028    & 29693.16602 & 8561.875    & 289.479156 & 90.416664 & 0.516917 & 0.021208 & 0.516917 & 0.564125 & 35.015644 \\ \hline
C & 0.015971 & 14744.48535 & 7380.685547 & 249.542862 & 77.942856 & 2.164771 & 0.5622   & 2.164829 & 2.254543 & 49.066856 \\ \hline
D & 0.047805 & 22182.56055 & 8591.707031 & 290.487793 & 90.731705 & 0.955463 & 2.089927 & 0.955512 & 1.011781 & 43.456512 \\ \hline
E & 0.033533 & 12407.09961 & 6653.799805 & 224.96666  & 70.26667  & 0.945433 & 1.299933 & 0.9455   & 1.002933 & 56.644001 \\ \hline
F & 0.021182 & 14687.39356 & 7116.36377  & 240.606064 & 75.151512 & 2.490757 & 2.880212 & 2.490849 & 2.56397  & 53.642487 \\ \hline
G & 0.024212 & 12590.90918 & 7116.36377  & 240.606064 & 75.151512 & 2.097788 & 0.997849 & 2.097788 & 2.170788 & 51.814091 \\ \hline
H & 0.472769 & 11528.07715 & 5871        & 198.5      & 62        & 1.276885 & 0.318577 & 1.276923 & 1.322808 & 64.375961 \\ \hline
I & 0.028    & 10858.63867 & 7175.666504 & 242.611115 & 75.777779 & 2.319195 & 0.164028 & 2.319278 & 2.415361 & 49.175667 \\ \hline
J & 0.184943 & 21486.14258 & 7380.685547 & 249.542862 & 77.942856 & 2.061286 & 0.290429 & 2.061314 & 2.1414   & 48.794056 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC14 before tuning}
\label{results_tc14_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.020115 & 62194.66797 & 11742       & 501.949585 & 118        & 0.192363 & 0.021179 & 0.192394 & 0.194189 & 0.195367 \\ \hline
B & 0.028013 & 56497.32031 & 11742       & 501.953369 & 118        & 0.205968 & 0.029005 & 0.206037 & 0.207074 & 0.208006 \\ \hline
C & 0.004756 & 43348.76172 & 11742       & 501.942596 & 118        & 0.254602 & 0.013649 & 0.254656 & 0.263959 & 0.27223  \\ \hline
D & 0.01754  & 47940.11328 & 11742       & 501.94809  & 118        & 0.246648 & 0.01869  & 0.246721 & 0.248382 & 0.249612 \\ \hline
E & 0.005014 & 41433.00391 & 11742       & 501.950348 & 118        & 0.267606 & 0.01408  & 0.267665 & 0.277162 & 0.285528 \\ \hline
F & 0.004945 & 43368.67969 & 11739.90918 & 501.869293 & 117.978989 & 0.254148 & 0.013957 & 0.254247 & 0.263593 & 0.27189  \\ \hline
G & 0.005551 & 47390.875   & 11742       & 501.949005 & 118        & 0.227961 & 0.015854 & 0.228029 & 0.239059 & 0.249047 \\ \hline
H & 0.020341 & 44710.39844 & 11742       & 501.950653 & 118        & 0.263499 & 0.021508 & 0.263541 & 0.265465 & 0.266742 \\ \hline
I & 0.005045 & 41742.18359 & 11742       & 501.866486 & 117.977905 & 0.264999 & 0.014134 & 0.265111 & 0.274604 & 0.283046 \\ \hline
J & 0.032237 & 62011.65625 & 11742       & 501.947723 & 118        & 0.191228 & 0.033577 & 0.191266 & 0.192807 & 0.193995 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC15 before tuning}
\label{results_tc15_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.340213 & 8257.826172 & 11730.23438 & 501.339691 & 118        & 1.36538  & 0.531221 & 1.365437 & 1.531829 & 1.830516 \\ \hline
B & 0.034971 & 12095.40039 & 11742       & 501.850342 & 118        & 0.770803 & 0.17654  & 0.770899 & 0.914825 & 1.181145 \\ \hline
C & 0.027634 & 8160.665039 & 11742       & 501.8414   & 118        & 1.055008 & 0.185498 & 1.05425  & 1.226756 & 1.506746 \\ \hline
D & 0.289014 & 10514.98438 & 11742       & 501.846405 & 118        & 1.167743 & 0.462584 & 1.167833 & 1.329151 & 1.609664 \\ \hline
E & 0.027378 & 8218.579102 & 11742       & 501.843384 & 118        & 1.059135 & 0.185662 & 1.058348 & 1.225625 & 1.509194 \\ \hline
F & 0.022364 & 8316.642578 & 11731.87793 & 501.393951 & 117.898277 & 1.022973 & 0.187677 & 1.023064 & 1.192021 & 1.476339 \\ \hline
G & 0.020126 & 8962.051758 & 11742       & 501.828796 & 118        & 0.934746 & 0.179293 & 0.934823 & 1.098645 & 1.380445 \\ \hline
H & 0.441911 & 6006.353516 & 11683.77539 & 499.343811 & 118        & 2.069026 & 0.645061 & 2.069109 & 2.283316 & 2.605666 \\ \hline
I & 0.039189 & 7751.248047 & 11742       & 501.867828 & 118        & 1.136165 & 0.210912 & 1.136281 & 1.314614 & 1.601192 \\ \hline
J & 0.244803 & 11135.72363 & 11742       & 501.842957 & 118        & 1.078655 & 0.426397 & 1.078705 & 1.234622 & 1.517611 \\ \hline
\end{tabular} }
\end{table*}


\begin{table*}[]
\caption{Results for TC18 before tuning}
\label{results_tc18_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.019293 & 60225.92188 & 11738.89844 & 396.895142 & 124        & 0.180424 & 0.020203 & 0.180472 & 0.200928 & 0.202637 \\ \hline
B & 0.028007 & 53157.89063 & 11734.86621 & 396.75882  & 124        & 0.201172 & 0.029367 & 0.201236 & 0.221682 & 0.223546 \\ \hline
C & 0.004801 & 42564.10547 & 11742       & 397        & 124        & 0.242631 & 0.014366 & 0.242767 & 0.271225 & 0.279649 \\ \hline
D & 0.014409 & 46712.40234 & 11742       & 397        & 124        & 0.232744 & 0.015332 & 0.232821 & 0.252631 & 0.254377 \\ \hline
E & 0.00479  & 42623.89063 & 11742       & 397        & 124        & 0.243128 & 0.013958 & 0.24325  & 0.270935 & 0.279285 \\ \hline
F & 0.004605 & 43994.09375 & 11737.66211 & 396.853333 & 124        & 0.233621 & 0.013787 & 0.233751 & 0.261823 & 0.27013  \\ \hline
G & 0.005396 & 46249.87891 & 11737.97363 & 396.863861 & 124        & 0.216528 & 0.016403 & 0.216617 & 0.247287 & 0.257283 \\ \hline
H & 0.024845 & 46774.11719 & 11742       & 397        & 124        & 0.240828 & 0.025588 & 0.240914 & 0.261036 & 0.262604 \\ \hline
I & 0.004869 & 42543.89063 & 11737.4834  & 396.847321 & 123.952309 & 0.242976 & 0.014103 & 0.243102 & 0.270995 & 0.279492 \\ \hline
J & 0.032789 & 58923.96875 & 11738.81152 & 396.892212 & 124        & 0.185032 & 0.03347  & 0.185072 & 0.204127 & 0.205782 \\ \hline
\end{tabular} }
\caption{Results for TC18}
\label{results_tc18}
\end{table*}

\begin{table*}[]
\caption{Results for TC19 before tuning}
\label{results_tc19_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.022756 & 32821.96484 & 11737.55078 & 396.849579 & 123.953011 & 0.420519 & 0.054385 & 0.420473 & 0.563559 & 0.65878  \\ \hline
B & 0.028035 & 31139.11719 & 11737.33106 & 396.842133 & 123.950699 & 0.439933 & 0.04509  & 0.440003 & 0.58818  & 0.687048 \\ \hline
C & 0.011461 & 24325.25586 & 11723.53809 & 396.375793 & 123.805031 & 0.490483 & 0.031592 & 0.490622 & 0.644817 & 0.828277 \\ \hline
D & 0.019447 & 28145.87891 & 11737.07715 & 396.833557 & 123.948006 & 0.473768 & 0.053924 & 0.473855 & 0.623012 & 0.726451 \\ \hline
E & 0.011898 & 24212.84961 & 11729.73633 & 396.585388 & 123.870499 & 0.553785 & 0.054419 & 0.553932 & 0.712399 & 0.830077 \\ \hline
F & 0.006669 & 26799.12109 & 11731.15332 & 396.63327  & 123.885452 & 0.445243 & 0.024845 & 0.44537  & 0.60379  & 0.771398 \\ \hline
G & 0.012083 & 27614.77344 & 11736.46387 & 396.812836 & 123.941536 & 0.49808  & 0.075417 & 0.498157 & 0.650564 & 0.75882  \\ \hline
H & 0.034107 & 23120.46289 & 11735.87793 & 396.792999 & 123.935349 & 0.578881 & 0.093225 & 0.578979 & 0.738059 & 0.857449 \\ \hline
I & 0.007579 & 26166.95508 & 11736.52344 & 396.814819 & 123.942162 & 0.505028 & 0.046531 & 0.505162 & 0.663324 & 0.774317 \\ \hline
J & 0.030267 & 34310.60156 & 11737.65625 & 396.853119 & 123.954124 & 0.410355 & 0.059561 & 0.410398 & 0.553371 & 0.6474   \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC20 before tuning}
\label{results_tc20_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.014341 & 58309.9375  & 11729.20898 & 497.259033 & 117.897171 & 0.200236 & 0.015643 & 0.200278 & 0.202193 & 0.203155 \\ \hline
B & 0.028    & 57137.01563 & 11725.56641 & 497.099609 & 117.862373 & 0.203484 & 0.028994 & 0.203511 & 0.204654 & 0.205273 \\ \hline
C & 0.004954 & 44078.00781 & 11720.31543 & 496.885803 & 117.854721 & 0.2506   & 0.013957 & 0.250719 & 0.260073 & 0.268345 \\ \hline
D & 0.015503 & 48502.86719 & 11726.12793 & 497.111115 & 117.904297 & 0.241705 & 0.016509 & 0.241774 & 0.243328 & 0.244321 \\ \hline
E & 0.00519  & 42452.80859 & 11723.1582  & 497.011871 & 117.886391 & 0.26077  & 0.014328 & 0.260834 & 0.270235 & 0.278604 \\ \hline
F & 0.004716 & 45191.86328 & 11728.00488 & 497.05484  & 117.85936  & 0.243213 & 0.013777 & 0.243311 & 0.252698 & 0.261034 \\ \hline
G & 0.006003 & 48840.25391 & 11723.02539 & 497.009705 & 117.872879 & 0.220463 & 0.01635  & 0.220527 & 0.231495 & 0.241529 \\ \hline
H & 0.018507 & 45689.35938 & 11721.46582 & 496.949005 & 117.862434 & 0.258577 & 0.019776 & 0.258653 & 0.260429 & 0.261422 \\ \hline
I & 0.005427 & 41473.03906 & 11726.50391 & 497.141876 & 117.883209 & 0.267132 & 0.01468  & 0.267256 & 0.276866 & 0.285513 \\ \hline
J & 0.030655 & 62132.97656 & 11727.19922 & 497.175629 & 117.900841 & 0.18865  & 0.031407 & 0.188692 & 0.19024  & 0.1912   \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC21 before tuning}
\label{results_tc21_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.068964 & 55690.34375 & 11742       & 500.463654 & 118 & 0.291737 & 0.082238 & 0.291787 & 0.300865 & 0.312276 \\ \hline
B & 0.04071  & 48872.01953 & 11742       & 500.305145 & 118 & 0.249366 & 0.04903  & 0.249433 & 0.258767 & 0.273809 \\ \hline
C & 0.012136 & 37919.80078 & 11742       & 500.417999 & 118 & 0.331486 & 0.031305 & 0.331602 & 0.349638 & 0.367839 \\ \hline
D & 0.093904 & 38641.80078 & 11742       & 500.39267  & 118 & 0.381017 & 0.108879 & 0.381109 & 0.391742 & 0.407276 \\ \hline
E & 0.011802 & 36455.53125 & 11742       & 500.405304 & 118 & 0.336256 & 0.028871 & 0.336372 & 0.354912 & 0.374287 \\ \hline
F & 0.01087  & 37726.29297 & 11742       & 500.411041 & 118 & 0.326415 & 0.030176 & 0.32652  & 0.346393 & 0.366749 \\ \hline
G & 0.012572 & 40000.26563 & 11742       & 500.410767 & 118 & 0.308993 & 0.032168 & 0.309062 & 0.330024 & 0.350814 \\ \hline
H & 0.086221 & 37405.98047 & 11742       & 500.463989 & 118 & 0.426654 & 0.102479 & 0.426682 & 0.43697  & 0.449293 \\ \hline
I & 0.021803 & 35802.99609 & 11742       & 500.391174 & 118 & 0.353976 & 0.040418 & 0.354098 & 0.373446 & 0.393639 \\ \hline
J & 0.071201 & 53370.94531 & 11739.99023 & 500.34491  & 118 & 0.272788 & 0.086979 & 0.272828 & 0.283183 & 0.296794 \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC22 before tuning}
\label{results_tc22_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.016235 & 62523.93359 & 11742       & 500.680176 & 117.986313 & 0.188493 & 0.017258 & 0.188548 & 0.190152 & 0.190908 \\ \hline
B & 0.028025 & 57322.53906 & 11742       & 500.679871 & 118        & 0.203324 & 0.029013 & 0.203364 & 0.204289 & 0.2049   \\ \hline
C & 0.004918 & 42840.45313 & 11739.92578 & 500.599091 & 117.979156 & 0.258386 & 0.01391  & 0.258495 & 0.267569 & 0.275848 \\ \hline
D & 0.018143 & 48220.06641 & 11742       & 500.684113 & 118        & 0.245875 & 0.019264 & 0.245946 & 0.247225 & 0.248126 \\ \hline
E & 0.005063 & 43041.34375 & 11742       & 500.674194 & 118        & 0.257357 & 0.014125 & 0.257471 & 0.266589 & 0.27494  \\ \hline
F & 0.004793 & 45082.66016 & 11742       & 500.687958 & 118        & 0.244508 & 0.01383  & 0.24462  & 0.253679 & 0.262001 \\ \hline
G & 0.006339 & 47189.92188 & 11742       & 500.683594 & 118        & 0.229855 & 0.016726 & 0.22989  & 0.240695 & 0.250738 \\ \hline
H & 0.02028  & 45725.02734 & 11742       & 500.676727 & 118        & 0.260411 & 0.02123  & 0.260492 & 0.262018 & 0.262962 \\ \hline
I & 0.012978 & 41760.20703 & 11742       & 500.66449  & 118        & 0.272946 & 0.022405 & 0.273014 & 0.282621 & 0.29142  \\ \hline
J & 0.032245 & 62336.39453 & 11742       & 500.6763   & 118        & 0.190522 & 0.033311 & 0.190562 & 0.191841 & 0.19267  \\ \hline
\end{tabular} }
\end{table*}

\begin{table*}[]
\caption{Results for TC23 before tuning}
\label{results_tc23_bf}
\resizebox{\textwidth}{!}{ \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
ID &
  \multicolumn{1}{l|}{Lookup time} &
  \multicolumn{1}{l|}{Download speed} &
  \multicolumn{1}{l|}{Size Download} &
  \multicolumn{1}{l|}{Header Size} &
  \multicolumn{1}{l|}{Request Size} &
  \multicolumn{1}{l|}{App conn time} &
  \multicolumn{1}{l|}{Conn time } &
  \multicolumn{1}{l|}{Pre transfer } &
  \multicolumn{1}{l|}{Start transfer} &
  \multicolumn{1}{l|}{Time} \\ \hline
A & 0.032456 & 58487.58594 & 11740.62988 & 500.600708 & 118        & 0.238117 & 0.040948 & 0.238175 & 0.244805 & 0.254168 \\ \hline
B & 0.04302  & 51359.41016 & 11742       & 500.657654 & 118        & 0.242575 & 0.049136 & 0.242628 & 0.24959  & 0.261084 \\ \hline
C & 0.011445 & 39702.35938 & 11742       & 500.665436 & 118        & 0.330751 & 0.033481 & 0.330871 & 0.347802 & 0.365594 \\ \hline
D & 0.02911  & 43205.52344 & 11742       & 500.666626 & 118        & 0.293325 & 0.04106  & 0.293395 & 0.301226 & 0.313982 \\ \hline
E & 0.008601 & 39221.67188 & 11739.98731 & 500.567017 & 117.979774 & 0.30985  & 0.026888 & 0.309957 & 0.326395 & 0.348524 \\ \hline
F & 0.009166 & 40093.44922 & 11742       & 500.664886 & 118        & 0.315406 & 0.031505 & 0.315463 & 0.331211 & 0.347473 \\ \hline
G & 0.008819 & 41766.10156 & 11742       & 500.662079 & 118        & 0.279098 & 0.029201 & 0.279176 & 0.29651  & 0.316196 \\ \hline
H & 0.034602 & 44148.99609 & 11738.40332 & 500.511566 & 117.981926 & 0.305516 & 0.045171 & 0.305604 & 0.312865 & 0.322424 \\ \hline
I & 0.011835 & 37385.64063 & 11739.75684 & 500.561981 & 117.977463 & 0.335938 & 0.030722 & 0.336067 & 0.352669 & 0.376666 \\ \hline
J & 0.044108 & 56492.02734 & 11742       & 500.655334 & 118        & 0.230668 & 0.054705 & 0.230714 & 0.237998 & 0.249817 \\ \hline
\end{tabular} }
\end{table*}

==> loadtest_2.tex <==
\begin{table*}[]
\caption{Results for TC0 after tuning}
\label{results_tc0_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time} & \multicolumn{1}{l|}{Conn time} & \multicolumn{1}{l|}{Pre transfer} & \multicolumn{1}{l|}{Start transfer} & \multicolumn{1}{l|}{Time} \\ \hline
A  & 0.10765                          & 299715.0625                         & 11742                              & 397                              & 124                               & 0                                  & 0.10774                        & 0.107743                          & 0.116995                            & 0.117044                  \\ \hline
B  & 0.028007                         & 303402.4375                         & 11742                              & 397                              & 123.991928                        & 0                                  & 0.029666                       & 0.029673                          & 0.039327                            & 0.039455                  \\ \hline
C  & 0.039049                         & 209277.9688                         & 11742                              & 397                              & 124                               & 0                                  & 0.048028                       & 0.048137                          & 0.066085                            & 0.066308                  \\ \hline
D  & 0.096488                         & 305289.9063                         & 11742                              & 397                              & 124                               & 0                                  & 0.097115                       & 0.097116                          & 0.106006                            & 0.10607                   \\ \hline
E  & 0.040415                         & 204297.125                          & 11742                              & 397                              & 123.986794                        & 0                                  & 0.049519                       & 0.049687                          & 0.067847                            & 0.068296                  \\ \hline
F  & 0.042825                         & 209526.125                          & 11742                              & 397                              & 124                               & 0                                  & 0.052306                       & 0.052434                          & 0.070326                            & 0.070588                  \\ \hline
G  & 0.05625                          & 197519.0313                         & 11742                              & 397                              & 124                               & 0                                  & 0.067622                       & 0.067663                          & 0.087348                            & 0.087627                  \\ \hline
H  & 0.094761                         & 301850.4063                         & 11742                              & 397                              & 124                               & 0                                  & 0.094821                       & 0.094822                          & 0.104054                            & 0.104111                  \\ \hline
I  & 0.034882                         & 40178.30469                         & 11742                              & 397                              & 124                               & 0.273846                           & 0.044552                       & 0.273989                          & 0.293171                            & 0.299291                  \\ \hline
J  & 0.032298                         & 311329.6875                         & 11742                              & 397                              & 123.992722                        & 0                                  & 0.033161                       & 0.033185                          & 0.041944                            & 0.041999                  \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC1 after tuning}
\label{results_tc1_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.067637                         & 145203.6875                         & 11742                              & 397                              & 124                               & 0                                      & 0.067831                           & 0.067837                              & 0.125331                                & 0.125383                      \\ \hline
B  & 0.028009                         & 145929.1875                         & 11742                              & 397                              & 124                               & 0                                      & 0.029539                           & 0.029562                              & 0.089791                                & 0.09001                       \\ \hline
C  & 0.039765                         & 118106.8594                         & 11740.2041                         & 396.939301                       & 123.981033                        & 0                                      & 0.04956                            & 0.049679                              & 0.118349                                & 0.118649                      \\ \hline
D  & 0.061503                         & 145939.3906                         & 11742                              & 397                              & 124                               & 0                                      & 0.062224                           & 0.062221                              & 0.121291                                & 0.121366                      \\ \hline
E  & 0.04205                          & 115116.9375                         & 11742                              & 397                              & 124                               & 0                                      & 0.052436                           & 0.052595                              & 0.11983                                 & 0.120133                      \\ \hline
F  & 0.042369                         & 117443.1563                         & 11742                              & 396.938538                       & 123.980797                        & 0                                      & 0.052442                           & 0.052565                              & 0.120164                                & 0.120453                      \\ \hline
G  & 0.044978                         & 114642.3594                         & 11740.26953                        & 396.941498                       & 123.981728                        & 0                                      & 0.056354                           & 0.056392                              & 0.127184                                & 0.127475                      \\ \hline
H  & 0.059853                         & 143400.4375                         & 11742                              & 397                              & 124                               & 0                                      & 0.059905                           & 0.059911                              & 0.119873                                & 0.119946                      \\ \hline
I  & 0.034539                         & 31739.08398                         & 11737.38672                        & 396.843994                       & 123.951279                        & 0.304247                               & 0.045303                           & 0.304393                              & 0.369301                                & 0.378297                      \\ \hline
J  & 0.034022                         & 149101.1875                         & 11742                              & 397                              & 124                               & 0                                      & 0.034971                           & 0.034984                              & 0.094316                                & 0.094377                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC2 after tuning}
\label{results_tc2_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.116203                         & 368656.1875                         & 11740.61231                        & 496.673401                       & 117.986053                        & 0                                      & 0.117548                           & 0.117647                              & 0.118984                                & 0.119065                      \\ \hline
B  & 0.02801                          & 401086.4375                         & 11742                              & 496.741028                       & 118                               & 0                                      & 0.029002                           & 0.029003                              & 0.029019                                & 0.029046                      \\ \hline
C  & 0.039732                         & 252284.1875                         & 11742                              & 496.72818                        & 118                               & 0                                      & 0.048287                           & 0.04835                               & 0.057011                                & 0.057301                      \\ \hline
D  & 0.104565                         & 374345.5938                         & 11742                              & 496.743042                       & 118                               & 0                                      & 0.105981                           & 0.106103                              & 0.107341                                & 0.107514                      \\ \hline
E  & 0.040403                         & 246212.7344                         & 11742                              & 496.738037                       & 118                               & 0                                      & 0.04921                            & 0.049322                              & 0.058276                                & 0.058566                      \\ \hline
F  & 0.042676                         & 249357.9375                         & 11742                              & 496.73941                        & 118                               & 0                                      & 0.051287                           & 0.051349                              & 0.06012                                 & 0.060389                      \\ \hline
G  & 0.067534                         & 235360.8125                         & 11740.79395                        & 496.692596                       & 117.987877                        & 0                                      & 0.078744                           & 0.078808                              & 0.089003                                & 0.089184                      \\ \hline
H  & 0.085421                         & 371751.2188                         & 11742                              & 496.733704                       & 118                               & 0                                      & 0.086837                           & 0.086939                              & 0.08822                                 & 0.088297                      \\ \hline
I  & 0.044008                         & 238947.6719                         & 11742                              & 496.729584                       & 118                               & 0                                      & 0.054079                           & 0.054224                              & 0.063682                                & 0.063994                      \\ \hline
J  & 0.030642                         & 382722.1875                         & 11742                              & 496.738342                       & 118                               & 0                                      & 0.032001                           & 0.032072                              & 0.033333                                & 0.033471                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC3 after tuning}
\label{results_tc3_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.146231                         & 20884.95508                         & 11742                              & 497.913757                       & 118                               & 0                                      & 0.427179                           & 0.427258                              & 0.648401                                & 1.001198                      \\ \hline
B  & 0.028009                         & 35605.76563                         & 11742                              & 497.887848                       & 118                               & 0                                      & 0.249395                           & 0.249489                              & 0.447604                                & 0.766879                      \\ \hline
C  & 0.03911                          & 17577.25391                         & 11742                              & 497.902496                       & 118                               & 0                                      & 0.312375                           & 0.312513                              & 0.539352                                & 0.887114                      \\ \hline
D  & 0.147004                         & 29269.55664                         & 11742                              & 497.876343                       & 118                               & 0                                      & 0.443464                           & 0.443536                              & 0.661681                                & 1.004843                      \\ \hline
E  & 0.044525                         & 17732.80273                         & 11742                              & 497.902771                       & 118                               & 0                                      & 0.302281                           & 0.30242                               & 0.534231                                & 0.88254                       \\ \hline
F  & 0.041005                         & 17342.20508                         & 11742                              & 497.925354                       & 118                               & 0                                      & 0.310395                           & 0.310512                              & 0.545381                                & 0.896785                      \\ \hline
G  & 0.036223                         & 19518.44531                         & 11742                              & 497.902679                       & 118                               & 0                                      & 0.304416                           & 0.304496                              & 0.524989                                & 0.864168                      \\ \hline
H  & 0.168334                         & 18560.92578                         & 11742                              & 497.899994                       & 118                               & 0                                      & 0.444694                           & 0.444815                              & 0.664194                                & 1.019172                      \\ \hline
I  & 0.076361                         & 16309.88086                         & 11742                              & 497.902771                       & 118                               & 0                                      & 0.361308                           & 0.36146                               & 0.611714                                & 0.97024                       \\ \hline
J  & 0.122749                         & 35183.44922                         & 11742                              & 497.878754                       & 118                               & 0                                      & 0.411043                           & 0.411097                              & 0.627534                                & 0.968778                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC6 after tuning}
\label{results_tc6_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.122962                         & 298700.0313                         & 11742                              & 397                              & 124                               & 0                                      & 0.123179                           & 0.1232                                & 0.133059                                & 0.133141                      \\ \hline
B  & 0.028006                         & 302500.8125                         & 11742                              & 397                              & 124                               & 0                                      & 0.029867                           & 0.029903                              & 0.040155                                & 0.040306                      \\ \hline
C  & 0.035432                         & 210188.2813                         & 11742                              & 397                              & 124                               & 0                                      & 0.045173                           & 0.045271                              & 0.063434                                & 0.063812                      \\ \hline
D  & 0.088303                         & 305859.375                          & 11742                              & 397                              & 124                               & 0                                      & 0.089006                           & 0.089016                              & 0.098406                                & 0.09847                       \\ \hline
E  & 0.033706                         & 206180.9688                         & 11742                              & 397                              & 123.987251                        & 0                                      & 0.043384                           & 0.043541                              & 0.061963                                & 0.062299                      \\ \hline
F  & 0.045874                         & 209175.0313                         & 11742                              & 397                              & 124                               & 0                                      & 0.055513                           & 0.055651                              & 0.073926                                & 0.074258                      \\ \hline
G  & 0.073808                         & 197484.8125                         & 11740.5752                         & 396.951813                       & 123.984947                        & 0                                      & 0.085548                           & 0.085587                              & 0.105414                                & 0.105684                      \\ \hline
H  & 0.078407                         & 302724.4063                         & 11742                              & 397                              & 124                               & 0                                      & 0.078563                           & 0.078585                              & 0.088393                                & 0.088449                      \\ \hline
I  & 0.031144                         & 40812.83984                         & 11738.46289                        & 396.880432                       & 123.962654                        & 0.268727                               & 0.040492                           & 0.268867                              & 0.287963                                & 0.291605                      \\ \hline
J  & 0.031761                         & 311123                              & 11742                              & 397                              & 124                               & 0                                      & 0.032771                           & 0.032789                              & 0.041853                                & 0.041924                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC7 after tuning}
\label{results_tc7_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 1.67896                          & 49763.36328                         & 11677.58008                        & 396.125702                       & 124                               & 0                                      & 1.706753                           & 1.706809                              & 1.941898                                & 2.008173                      \\ \hline
B  & 0.028024                         & 58926.67578                         & 11670.72949                        & 396.031494                       & 124                               & 0                                      & 0.246364                           & 0.246457                              & 0.513585                                & 0.659237                      \\ \hline
C  & 0.040843                         & 44555.34766                         & 11700.8877                         & 396.443329                       & 124                               & 0                                      & 0.282338                           & 0.282466                              & 0.56904                                 & 0.689125                      \\ \hline
D  & 1.499186                         & 63897.85938                         & 11628.7959                         & 395.463593                       & 124                               & 0                                      & 1.522197                           & 1.522277                              & 1.723761                                & 1.769869                      \\ \hline
E  & 0.032921                         & 42916.48828                         & 11639.13281                        & 395.586792                       & 124                               & 0                                      & 0.290343                           & 0.290501                              & 0.590388                                & 0.734961                      \\ \hline
F  & 0.032915                         & 43657.5625                          & 11702.92969                        & 396.466034                       & 124                               & 0                                      & 0.258                              & 0.258117                              & 0.521686                                & 0.649974                      \\ \hline
G  & 0.046218                         & 41702.34375                         & 11688.94336                        & 396.072754                       & 123.93734                         & 0                                      & 0.304511                           & 0.304579                              & 0.589784                                & 0.708805                      \\ \hline
H  & 1.496822                         & 50696.59375                         & 11625.57129                        & 395.394012                       & 124                               & 0                                      & 1.525238                           & 1.525311                              & 1.735355                                & 1.789202                      \\ \hline
I  & 0.037667                         & 13996.31738                         & 11608.99609                        & 395.194855                       & 124                               & 0.879221                               & 0.25594                            & 0.879358                              & 1.257474                                & 1.341999                      \\ \hline
J  & 1.247882                         & 78833.97656                         & 11656.0127                         & 395.566772                       & 123.869614                        & 0                                      & 1.271957                           & 1.272009                              & 1.458364                                & 1.534731                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC8 after tuning}
\label{results_tc8_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.121152                         & 317083.4063                         & 11742                              & 498.704529                       & 118                               & 0                                      & 0.126362                           & 0.12642                               & 0.129896                                & 0.130925                      \\ \hline
B  & 0.028007                         & 357492.4375                         & 11742                              & 498.727112                       & 118                               & 0                                      & 0.030598                           & 0.030664                              & 0.032629                                & 0.033117                      \\ \hline
C  & 0.041317                         & 221385.7656                         & 11740.96191                        & 498.698975                       & 117.989563                        & 0                                      & 0.051658                           & 0.051771                              & 0.062223                                & 0.065592                      \\ \hline
D  & 0.098539                         & 322316.5313                         & 11742                              & 498.761169                       & 118                               & 0                                      & 0.102699                           & 0.102767                              & 0.10608                                 & 0.107098                      \\ \hline
E  & 0.042338                         & 217506.1719                         & 11742                              & 498.713287                       & 118                               & 0                                      & 0.052928                           & 0.05306                               & 0.06369                                 & 0.067101                      \\ \hline
F  & 0.041741                         & 221004.3438                         & 11740.96777                        & 498.702087                       & 117.989624                        & 0                                      & 0.052133                           & 0.052244                              & 0.062685                                & 0.066075                      \\ \hline
G  & 0.069422                         & 207286.4844                         & 11742                              & 498.674316                       & 117.987854                        & 0                                      & 0.081606                           & 0.081687                              & 0.09394                                 & 0.097337                      \\ \hline
H  & 0.085646                         & 317117.375                          & 11742                              & 498.713989                       & 117.987381                        & 0                                      & 0.090281                           & 0.090353                              & 0.093861                                & 0.094908                      \\ \hline
I  & 0.040539                         & 218907.75                           & 11742                              & 498.737823                       & 118                               & 0                                      & 0.051188                           & 0.05131                               & 0.061898                                & 0.065299                      \\ \hline
J  & 0.037918                         & 330787.0313                         & 11742                              & 498.714172                       & 118                               & 0                                      & 0.043065                           & 0.043112                              & 0.046336                                & 0.047362                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC9 after tuning}
\label{results_tc9_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.098253                         & 20289.54102                         & 11742                              & 499.84726                        & 118                               & 0                                      & 0.265381                           & 0.265462                              & 0.427985                                & 0.74953                       \\ \hline
B  & 0.033502                         & 28759.43164                         & 11736.14648                        & 499.506989                       & 117.941177                        & 0                                      & 0.189196                           & 0.189292                              & 0.34482                                 & 0.6546                        \\ \hline
C  & 0.041264                         & 20311.50977                         & 11742                              & 499.864563                       & 118                               & 0                                      & 0.213177                           & 0.213307                              & 0.381978                                & 0.701197                      \\ \hline
D  & 0.082821                         & 20711.39844                         & 11742                              & 499.85907                        & 118                               & 0                                      & 0.25351                            & 0.253581                              & 0.416711                                & 0.738841                      \\ \hline
E  & 0.041839                         & 19842.51953                         & 11742                              & 499.868866                       & 118                               & 0                                      & 0.212823                           & 0.212961                              & 0.383283                                & 0.703608                      \\ \hline
F  & 0.032192                         & 19807.03125                         & 11742                              & 499.876434                       & 118                               & 0                                      & 0.202582                           & 0.20272                               & 0.372227                                & 0.693343                      \\ \hline
G  & 0.032553                         & 20552.39844                         & 11742                              & 499.873871                       & 118                               & 0                                      & 0.204543                           & 0.204625                              & 0.374911                                & 0.694146                      \\ \hline
H  & 0.094832                         & 20246.43164                         & 11742                              & 499.579102                       & 117.927917                        & 0                                      & 0.264151                           & 0.264237                              & 0.42907                                 & 0.750191                      \\ \hline
I  & 0.043163                         & 19454.21094                         & 11742                              & 499.881744                       & 118                               & 0                                      & 0.216397                           & 0.216535                              & 0.387461                                & 0.70931                       \\ \hline
J  & 0.09828                          & 21789.10742                         & 11742                              & 499.879944                       & 118                               & 0                                      & 0.266704                           & 0.266771                              & 0.428656                                & 0.750028                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC10 after tuning}
\label{results_tc10_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.109053                         & 310066.3438                         & 11742                              & 500.948151                       & 118                               & 0                                      & 0.114703                           & 0.114764                              & 0.118507                                & 0.119811                      \\ \hline
B  & 0.028009                         & 360215.25                           & 11742                              & 500.948273                       & 118                               & 0                                      & 0.030494                           & 0.030559                              & 0.032412                                & 0.032861                      \\ \hline
C  & 0.045282                         & 222911.0781                         & 11742                              & 500.950348                       & 118                               & 0                                      & 0.055466                           & 0.055576                              & 0.0659                                  & 0.069109                      \\ \hline
D  & 0.109091                         & 316136.125                          & 11742                              & 500.948761                       & 118                               & 0                                      & 0.114804                           & 0.114869                              & 0.118306                                & 0.119398                      \\ \hline
E  & 0.048539                         & 217243.4063                         & 11742                              & 500.946198                       & 117.987122                        & 0                                      & 0.059087                           & 0.059221                              & 0.069819                                & 0.073001                      \\ \hline
F  & 0.041192                         & 222510.4844                         & 11742                              & 500.951019                       & 118                               & 0                                      & 0.051459                           & 0.051574                              & 0.061928                                & 0.065059                      \\ \hline
G  & 0.077574                         & 210076.7813                         & 11742                              & 500.946808                       & 118                               & 0                                      & 0.089679                           & 0.089758                              & 0.101769                                & 0.104879                      \\ \hline
H  & 0.094859                         & 310203.7813                         & 11742                              & 500.939819                       & 118                               & 0                                      & 0.100064                           & 0.100136                              & 0.103813                                & 0.105048                      \\ \hline
I  & 0.045027                         & 220924.6094                         & 11742                              & 500.954102                       & 118                               & 0                                      & 0.055358                           & 0.055478                              & 0.065903                                & 0.069094                      \\ \hline
J  & 0.050513                         & 325287.9063                         & 11742                              & 500.94104                        & 118                               & 0                                      & 0.056423                           & 0.05647                               & 0.059906                                & 0.061035                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC11 after tuning}
\label{results_tc11_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.17411                          & 19115.00977                         & 11742                              & 500.786865                       & 118                               & 0                                      & 0.36944                            & 0.369524                              & 0.544364                                & 0.877221                      \\ \hline
B  & 0.040811                         & 20336.81055                         & 11742                              & 500.777649                       & 118                               & 0                                      & 0.198448                           & 0.198554                              & 0.35551                                 & 0.66927                       \\ \hline
C  & 0.040568                         & 18661.69727                         & 11742                              & 500.810944                       & 118                               & 0                                      & 0.218807                           & 0.218941                              & 0.387952                                & 0.706972                      \\ \hline
D  & 0.247955                         & 19564.65039                         & 11742                              & 500.828735                       & 118                               & 0                                      & 0.430383                           & 0.430455                              & 0.59688                                 & 0.918507                      \\ \hline
E  & 0.058938                         & 18110.55273                         & 11742                              & 500.802032                       & 118                               & 0                                      & 0.229887                           & 0.23004                               & 0.400459                                & 0.720509                      \\ \hline
F  & 0.047221                         & 18554.41016                         & 11742                              & 500.808197                       & 118                               & 0                                      & 0.228322                           & 0.228449                              & 0.396933                                & 0.716511                      \\ \hline
G  & 0.03774                          & 18407.44727                         & 11742                              & 500.782867                       & 118                               & 0                                      & 0.209022                           & 0.209109                              & 0.380037                                & 0.700079                      \\ \hline
H  & 0.238769                         & 17983.19922                         & 11731.92969                        & 500.394501                       & 118                               & 0                                      & 0.429372                           & 0.429478                              & 0.61019                                 & 0.940805                      \\ \hline
I  & 0.049686                         & 18344.14844                         & 11742                              & 500.820557                       & 118                               & 0                                      & 0.219779                           & 0.21992                               & 0.389719                                & 0.719838                      \\ \hline
J  & 0.184146                         & 20149.44141                         & 11742                              & 500.816345                       & 118                               & 0                                      & 0.363277                           & 0.363335                              & 0.526633                                & 0.846268                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC12 after tuning}
\label{results_tc12_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.046509                         & 59324.42969                         & 11742                              & 397                              & 124                               & 0.195983                               & 0.046603                           & 0.196041                              & 0.213169                                & 0.213805                      \\ \hline
B  & 0.030416                         & 54052.91406                         & 11742                              & 397                              & 124                               & 0.203737                               & 0.032058                           & 0.203799                              & 0.222387                                & 0.223231                      \\ \hline
C  & 0.034157                         & 41076.43359                         & 11738.62598                        & 396.885925                       & 123.964371                        & 0.260509                               & 0.043517                           & 0.260635                              & 0.286311                                & 0.293313                      \\ \hline
D  & 0.038341                         & 43991.16016                         & 11742                              & 397                              & 124                               & 0.258883                               & 0.0388                             & 0.258958                              & 0.27519                                 & 0.275748                      \\ \hline
E  & 0.033781                         & 37778.83203                         & 11738.2627                         & 396.873657                       & 123.960533                        & 0.285702                               & 0.043257                           & 0.285855                              & 0.314414                                & 0.321503                      \\ \hline
F  & 0.034308                         & 40537.43359                         & 11742                              & 397                              & 124                               & 0.266227                               & 0.045239                           & 0.26635                               & 0.291825                                & 0.29896                       \\ \hline
G  & 0.028588                         & 44458.07813                         & 11742                              & 397                              & 124                               & 0.231495                               & 0.04012                            & 0.231573                              & 0.258673                                & 0.266938                      \\ \hline
H  & 0.045345                         & 46533.58984                         & 11742                              & 397                              & 124                               & 0.248955                               & 0.045471                           & 0.249029                              & 0.266138                                & 0.266747                      \\ \hline
I  & 0.033376                         & 38022.46875                         & 11742                              & 397                              & 124                               & 0.28374                                & 0.043295                           & 0.283893                              & 0.308942                                & 0.316035                      \\ \hline
J  & 0.032407                         & 59665.14453                         & 11742                              & 397                              & 124                               & 0.186089                               & 0.03324                            & 0.18613                               & 0.201693                                & 0.202251                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC13 after tuning}
\label{results_tc13_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.038                            & 8491.333008                         & 6523.333496                        & 220.555557                       & 68.888885                         & 0.599611                               & 3.530944                           & 0.599667                              & 0.666                                   & 66.779945                     \\ \hline
B  & 0.028                            & 15219.26074                         & 7147.304199                        & 241.652176                       & 75.478264                         & 0.584348                               & 2.765261                           & 0.584348                              & 0.646304                                & 52.331654                     \\ \hline
C  & 0.045778                         & 7516.944336                         & 5871                               & 198.5                            & 62                                & 0.7935                                 & 0.035278                           & 0.7935                                & 0.857167                                & 64.468613                     \\ \hline
D  & 0.03592                          & 14342.91992                         & 7514.879883                        & 254.080002                       & 79.360001                         & 4.14224                                & 2.70924                            & 4.14228                               & 4.215                                   & 49.243999                     \\ \hline
E  & 0.04345                          & 7119.299805                         & 6458.100098                        & 218.350006                       & 68.199997                         & 2.10545                                & 7.10665                            & 2.10565                               & 2.1839                                  & 63.258598                     \\ \hline
F  & 0.042                            & 7435.388672                         & 5871                               & 198.5                            & 62                                & 2.345667                               & 0.368056                           & 2.345667                              & 2.448056                                & 64.50322                      \\ \hline
G  & 0.03975                          & 7346.350098                         & 6458.100098                        & 218.350006                       & 68.199997                         & 1.0473                                 & 3.3987                             & 1.0473                                & 1.11985                                 & 58.862949                     \\ \hline
H  & 0.049095                         & 8922.428711                         & 6709.714355                        & 226.857147                       & 70.85714                          & 1.422286                               & 0.171429                           & 1.422476                              & 1.496286                                & 56.023903                     \\ \hline
I  & 0.048778                         & 5274.666504                         & 6523.333496                        & 220.555557                       & 68.888885                         & 7.635334                               & 5.275667                           & 7.635389                              & 7.758056                                & 66.93589                      \\ \hline
J  & 0.028034                         & 13864.31055                         & 8097.931152                        & 273.793091                       & 85.517242                         & 5.309345                               & 1.680172                           & 5.309345                              & 5.442207                                & 43.481346                     \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC14 after tuning}
\label{results_tc14_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.047081                         & 60383.50781                         & 11742                              & 500.753204                       & 118                               & 0.208612                               & 0.048339                           & 0.208667                              & 0.210799                                & 0.212028                      \\ \hline
B  & 0.028006                         & 55999.375                           & 11742                              & 500.752594                       & 118                               & 0.207801                               & 0.029                              & 0.207861                              & 0.209077                                & 0.209956                      \\ \hline
C  & 0.044569                         & 40603.31641                         & 11742                              & 500.76297                        & 118                               & 0.286762                               & 0.053037                           & 0.286858                              & 0.296194                                & 0.304425                      \\ \hline
D  & 0.047634                         & 43580.29297                         & 11742                              & 500.744232                       & 118                               & 0.285038                               & 0.048982                           & 0.285102                              & 0.286907                                & 0.288204                      \\ \hline
E  & 0.039416                         & 40343.89453                         & 11738.56641                        & 500.587128                       & 117.9655                          & 0.28391                                & 0.047913                           & 0.284014                              & 0.293353                                & 0.301616                      \\ \hline
F  & 0.039358                         & 40846.46094                         & 11742                              & 500.74588                        & 118                               & 0.280156                               & 0.047868                           & 0.280256                              & 0.289728                                & 0.298017                      \\ \hline
G  & 0.031337                         & 45470.62891                         & 11739.10742                        & 500.62561                        & 117.97094                         & 0.240585                               & 0.04177                            & 0.24064                               & 0.251664                                & 0.261638                      \\ \hline
H  & 0.037871                         & 44804.20703                         & 11742                              & 500.608612                       & 117.968193                        & 0.267458                               & 0.039357                           & 0.267541                              & 0.269753                                & 0.271024                      \\ \hline
I  & 0.041897                         & 38727.53906                         & 11742                              & 500.757629                       & 118                               & 0.298022                               & 0.050516                           & 0.298137                              & 0.30757                                 & 0.315926                      \\ \hline
J  & 0.034492                         & 59667.71094                         & 11742                              & 500.744873                       & 118                               & 0.201569                               & 0.036854                           & 0.201613                              & 0.203473                                & 0.20469                       \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC15 after tuning}
\label{results_tc15_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.35707                          & 7803.44043                          & 11742                              & 501.820343                       & 118                               & 1.412992                               & 0.576727                           & 1.413062                              & 1.577758                                & 1.87939                       \\ \hline
B  & 0.028016                         & 12360.51758                         & 11742                              & 501.818634                       & 118                               & 0.783515                               & 0.181574                           & 0.783585                              & 0.923822                                & 1.188147                      \\ \hline
C  & 0.086548                         & 7777.142578                         & 11742                              & 501.814972                       & 118                               & 1.100523                               & 0.261093                           & 1.100631                              & 1.265544                                & 1.555208                      \\ \hline
D  & 0.439214                         & 9289.480469                         & 11742                              & 501.795013                       & 118                               & 1.342854                               & 0.627902                           & 1.342925                              & 1.499444                                & 1.782461                      \\ \hline
E  & 0.09305                          & 7701.704102                         & 11708.45117                        & 500.391418                       & 117.831429                        & 1.117403                               & 0.259847                           & 1.117503                              & 1.287387                                & 1.578319                      \\ \hline
F  & 0.082823                         & 8205.996094                         & 11742                              & 501.793243                       & 118                               & 1.063078                               & 0.252081                           & 1.063172                              & 1.226385                                & 1.507088                      \\ \hline
G  & 0.048291                         & 8908.886719                         & 11742                              & 501.813782                       & 118                               & 0.951703                               & 0.214641                           & 0.951776                              & 1.113022                                & 1.396486                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.086838                         & 7970.237793                         & 11725.46191                        & 501.121124                       & 117.833801                        & 1.101108                               & 0.250776                           & 1.101217                              & 1.268172                                & 1.5534                        \\ \hline
J  & 0.33687                          & 10613.62598                         & 11726.13281                        & 501.125671                       & 118                               & 1.214724                               & 0.544958                           & 1.214772                              & 1.375362                                & 1.650916                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC18 after tuning}
\label{results_tc18_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.044639                         & 57777.29297                         & 11742                              & 397                              & 124                               & 0.199848                               & 0.044795                           & 0.199905                              & 0.217248                                & 0.21818                       \\ \hline
B  & 0.028006                         & 53953.33203                         & 11742                              & 397                              & 124                               & 0.201666                               & 0.030277                           & 0.201728                              & 0.219097                                & 0.220068                      \\ \hline
C  & 0.033054                         & 38811.60156                         & 11742                              & 397                              & 124                               & 0.274838                               & 0.042663                           & 0.274965                              & 0.300516                                & 0.308592                      \\ \hline
D  & 0.030923                         & 43428.54297                         & 11742                              & 397                              & 124                               & 0.255092                               & 0.031528                           & 0.255162                              & 0.272638                                & 0.273538                      \\ \hline
E  & 0.032797                         & 39234.98047                         & 11738.67383                        & 396.887543                       & 123.964874                        & 0.271352                               & 0.042438                           & 0.271473                              & 0.297152                                & 0.305357                      \\ \hline
F  & 0.033114                         & 39242.30078                         & 11742                              & 397                              & 124                               & 0.270677                               & 0.042744                           & 0.270801                              & 0.296887                                & 0.30534                       \\ \hline
G  & 0.031502                         & 42824.78125                         & 11742                              & 397                              & 124                               & 0.242036                               & 0.042309                           & 0.242118                              & 0.26954                                 & 0.279485                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.038657                         & 38076.58594                         & 11738.51953                        & 396.882324                       & 123.963249                        & 0.284776                               & 0.047611                           & 0.28491                               & 0.311073                                & 0.319201                      \\ \hline
J  & 0.031169                         & 58410.91406                         & 11742                              & 397                              & 124                               & 0.187668                               & 0.032048                           & 0.187717                              & 0.204357                                & 0.205281                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC19 after tuning}
\label{results_tc19_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 1.815939                         & 7984.039551                         & 11742                              & 397                              & 124                               & 2.47743                                & 1.826362                           & 2.477499                              & 2.949667                                & 3.274169                      \\ \hline
B  & 0.028042                         & 9743.496094                         & 11723.85156                        & 396.386414                       & 123.80835                         & 1.068403                               & 0.331369                           & 1.068485                              & 1.56011                                 & 2.010433                      \\ \hline
C  & 0.075415                         & 7761.455078                         & 11742                              & 397                              & 124                               & 1.266104                               & 0.320756                           & 1.266208                              & 1.769846                                & 2.175009                      \\ \hline
D  & 2.22124                          & 10353.21289                         & 11742                              & 397                              & 124                               & 2.755175                               & 2.221749                           & 2.755261                              & 3.254259                                & 3.536749                      \\ \hline
E  & 0.085086                         & 7540.192383                         & 11742                              & 397                              & 124                               & 1.261645                               & 0.337047                           & 1.261764                              & 1.771196                                & 2.193308                      \\ \hline
F  & 0.05637                          & 7319.6875                           & 11742                              & 397                              & 124                               & 1.213675                               & 0.307117                           & 1.213769                              & 1.737784                                & 2.172541                      \\ \hline
G  & 0.050893                         & 7952.11084                          & 11722.29883                        & 396.333893                       & 123.791946                        & 1.185294                               & 0.30274                            & 1.185367                              & 1.706245                                & 2.140634                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.108906                         & 7405.003906                         & 11719.5918                         & 396.242371                       & 123.763359                        & 1.400635                               & 0.397145                           & 1.40075                               & 1.925076                                & 2.372691                      \\ \hline
J  & 1.605437                         & 11368.0459                          & 11715.25293                        & 396.095673                       & 123.717537                        & 2.097303                               & 1.606558                           & 2.097339                              & 2.554706                                & 2.92649                       \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC20 after tuning}
\label{results_tc20_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.057733                         & 52590.73828                         & 11742                              & 498.425934                       & 118                               & 0.242454                               & 0.059412                           & 0.242518                              & 0.245388                                & 0.247385                      \\ \hline
B  & 0.028015                         & 55625.87109                         & 11742                              & 498.431915                       & 118                               & 0.208716                               & 0.029007                           & 0.208786                              & 0.210272                                & 0.211366                      \\ \hline
C  & 0.043405                         & 38375.66797                         & 11742                              & 498.467133                       & 118                               & 0.301444                               & 0.052007                           & 0.301553                              & 0.311235                                & 0.319555                      \\ \hline
D  & 0.046675                         & 44012.375                           & 11742                              & 498.415375                       & 118                               & 0.280012                               & 0.048432                           & 0.280038                              & 0.282457                                & 0.284235                      \\ \hline
E  & 0.044299                         & 38735.38281                         & 11742                              & 498.414734                       & 118                               & 0.299418                               & 0.052961                           & 0.299448                              & 0.309213                                & 0.317485                      \\ \hline
F  & 0.046672                         & 39293.33984                         & 11742                              & 498.44458                        & 117.966713                        & 0.297359                               & 0.055274                           & 0.297458                              & 0.307017                                & 0.315345                      \\ \hline
G  & 0.033059                         & 43397.3125                          & 11742                              & 498.290527                       & 117.971313                        & 0.258155                               & 0.047159                           & 0.258227                              & 0.269552                                & 0.279592                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.0579                           & 35526.03906                         & 11742                              & 498.473114                       & 118                               & 0.339059                               & 0.069975                           & 0.339183                              & 0.349865                                & 0.358972                      \\ \hline
J  & 0.030094                         & 57875.92969                         & 11742                              & 498.422455                       & 118                               & 0.202875                               & 0.03289                            & 0.202918                              & 0.205184                                & 0.206927                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC21 after tuning}
\label{results_tc21_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.894368                         & 6970.936523                         & 11658.91992                        & 495.04953                        & 117.721695                        & 2.141484                               & 1.138863                           & 2.141538                              & 2.351189                                & 2.694182                      \\ \hline
B  & 0.033189                         & 12356.10645                         & 11742                              & 498.438599                       & 118                               & 0.769806                               & 0.16748                            & 0.769878                              & 0.916205                                & 1.1912                        \\ \hline
C  & 0.102406                         & 7579.007324                         & 11742                              & 498.616302                       & 118                               & 1.168664                               & 0.257739                           & 1.168757                              & 1.341535                                & 1.635483                      \\ \hline
D  & 0.639094                         & 8022.671875                         & 11722.23242                        & 497.819855                       & 118                               & 1.6413                                 & 0.845463                           & 1.641397                              & 1.83482                                 & 2.176845                      \\ \hline
E  & 0.077719                         & 7801.708496                         & 11742                              & 498.55249                        & 118                               & 1.143136                               & 0.231843                           & 1.143241                              & 1.315901                                & 1.605047                      \\ \hline
F  & 0.088172                         & 7754.935059                         & 11742                              & 498.560059                       & 118                               & 1.139159                               & 0.242088                           & 1.139275                              & 1.310096                                & 1.602945                      \\ \hline
G  & 0.045875                         & 8900.506836                         & 11742                              & 498.496857                       & 118                               & 0.99461                                & 0.201546                           & 0.99468                               & 1.162849                                & 1.447641                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.356673                         & 6354.593262                         & 11718.70215                        & 497.664673                       & 117.765877                        & 1.631673                               & 0.547038                           & 1.631774                              & 1.843522                                & 2.138974                      \\ \hline
J  & 0.516642                         & 8869.533203                         & 11742                              & 498.590912                       & 118                               & 1.452288                               & 0.7241                             & 1.452345                              & 1.642395                                & 1.964673                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC22 after tuning}
\label{results_tc22_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.063536                         & 53110.67969                         & 11742                              & 499.911407                       & 118                               & 0.245477                               & 0.066303                           & 0.24554                               & 0.248158                                & 0.249992                      \\ \hline
B  & 0.028014                         & 55510.45313                         & 11742                              & 499.905121                       & 118                               & 0.208884                               & 0.029007                           & 0.208957                              & 0.210549                                & 0.211867                      \\ \hline
C  & 0.033416                         & 39147.69531                         & 11742                              & 499.909058                       & 118                               & 0.286105                               & 0.041948                           & 0.286219                              & 0.296087                                & 0.30439                       \\ \hline
D  & 0.059045                         & 42649.90625                         & 11742                              & 499.903503                       & 118                               & 0.295486                               & 0.059841                           & 0.295563                              & 0.297918                                & 0.299696                      \\ \hline
E  & 0.045436                         & 38713.27344                         & 11742                              & 499.902191                       & 117.966835                        & 0.301409                               & 0.053995                           & 0.301506                              & 0.311222                                & 0.319542                      \\ \hline
F  & 0.034773                         & 38861.05859                         & 11742                              & 499.907043                       & 118                               & 0.289704                               & 0.043332                           & 0.28981                               & 0.299603                                & 0.307894                      \\ \hline
G  & 0.033258                         & 43369.83984                         & 11742                              & 499.910706                       & 118                               & 0.254754                               & 0.043714                           & 0.254825                              & 0.266222                                & 0.276288                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.056157                         & 35340.35938                         & 11738.25488                        & 499.752777                       & 117.962364                        & 0.337512                               & 0.065862                           & 0.337635                              & 0.348377                                & 0.35724                       \\ \hline
J  & 0.037149                         & 57498.22266                         & 11742                              & 499.905426                       & 118                               & 0.210251                               & 0.038759                           & 0.210295                              & 0.212711                                & 0.214395                      \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\caption{Results for TC23 after tuning}
\label{results_tc23_af}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\hline
ID & \multicolumn{1}{l|}{Lookup time} & \multicolumn{1}{l|}{Download speed} & \multicolumn{1}{l|}{size download} & \multicolumn{1}{l|}{Header size} & \multicolumn{1}{l|}{Request size} & \multicolumn{1}{l|}{App conn time (S)} & \multicolumn{1}{l|}{Conn time (S)} & \multicolumn{1}{l|}{Pre transfer (S)} & \multicolumn{1}{l|}{Start transfer (S)} & \multicolumn{1}{l|}{Time (S)} \\ \hline
A  & 0.301887                         & 7322.029297                         & 11742                              & 500.650269                       & 118                               & 1.388417                               & 0.47247                            & 1.388477                              & 1.566566                                & 1.886102                      \\ \hline
B  & 0.033683                         & 10623.19531                         & 11742                              & 500.613098                       & 118                               & 0.813872                               & 0.18062                            & 0.813957                              & 0.973608                                & 1.269982                      \\ \hline
C  & 0.07948                          & 7473.799316                         & 11742                              & 500.644684                       & 118                               & 1.15516                                & 0.246792                           & 1.155246                              & 1.335187                                & 1.644288                      \\ \hline
D  & 0.213517                         & 9621.334961                         & 11742                              & 500.625305                       & 118                               & 1.069908                               & 0.377284                           & 1.06999                               & 1.235521                                & 1.53714                       \\ \hline
E  & 0.077606                         & 7577.475586                         & 11724.55273                        & 499.894501                       & 117.824669                        & 1.137657                               & 0.242391                           & 1.137762                              & 1.318299                                & 1.626053                      \\ \hline
F  & 0.066898                         & 7676.483398                         & 11742                              & 500.655121                       & 118                               & 1.112433                               & 0.232253                           & 1.112535                              & 1.289089                                & 1.595072                      \\ \hline
G  & 0.042545                         & 8334.337891                         & 11727.15527                        & 500.006317                       & 117.850822                        & 0.988497                               & 0.205532                           & 0.988571                              & 1.164895                                & 1.471552                      \\ \hline
H  & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}         \\ \hline
I  & 0.102632                         & 6709.590332                         & 11742                              & 500.63205                        & 118                               & 1.331898                               & 0.274095                           & 1.331996                              & 1.523117                                & 1.830178                      \\ \hline
J  & 0.101291                         & 10405.08106                         & 11742                              & 500.615997                       & 118                               & 0.924151                               & 0.261743                           & 0.924199                              & 1.091777                                & 1.393926                      \\ \hline
\end{tabular}
}
\end{table*}

==> tutorial.tex <==
%% bare_adv.tex
%% V1.4b
%% 2015/08/26
%% by Michael Shell
%% See: 
%% http://www.michaelshell.org/
%% for current contact information.
%%
%% This is a skeleton file demonstrating the advanced use of IEEEtran.cls
%% (requires IEEEtran.cls version 1.8b or later) with an IEEE Computer
%% Society journal paper.
%%
%% Support sites:
%% http://www.michaelshell.org/tex/ieeetran/
%% http://www.ctan.org/pkg/ieeetran
%% and
%% http://www.ieee.org/

%%*************************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE! 
%% User assumes all risk.
%% In no event shall the IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%
%% This work is distributed under the LaTeX Project Public License (LPPL)
%% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
%% distributed and modified. A copy of the LPPL, version 1.3, is included
%% in the base LaTeX documentation of all distributions of LaTeX released
%% 2003/12/01 or later.
%% Retain all contribution notices and credits.
%% ** Modified files should be clearly indicated as such, including  **
%% ** renaming them and changing author support contact information. **
%%*************************************************************************


% *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% *** with production work. The IEEE's font choices and paper sizes can   ***
% *** trigger bugs that do not appear when using other class files.       ***                          ***
% The testflow support page is at:
% http://www.michaelshell.org/tex/testflow/


% IEEEtran V1.7 and later provides for these CLASSINPUT macros to allow the
% user to reprogram some IEEEtran.cls defaults if needed. These settings
% override the internal defaults of IEEEtran.cls regardless of which class
% options are used. Do not use these unless you have good reason to do so as
% they can result in nonIEEE compliant documents. User beware. ;)
%
%\newcommand{\CLASSINPUTbaselinestretch}{1.0} % baselinestretch
%\newcommand{\CLASSINPUTinnersidemargin}{1in} % inner side margin
%\newcommand{\CLASSINPUToutersidemargin}{1in} % outer side margin
%\newcommand{\CLASSINPUTtoptextmargin}{1in}   % top text margin
%\newcommand{\CLASSINPUTbottomtextmargin}{1in}% bottom text margin




%

% If IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it like:
% \documentclass[10pt,journal,compsoc]{../sty/IEEEtran}


% For Computer Society journals, IEEEtran defaults to the use of 
% Palatino/Palladio as is done in IEEE Computer Society journals.
% To go back to Times Roman, you can use this code:
%\renewcommand{\rmdefault}{ptm}\selectfont





% Some very useful LaTeX packages include:
% (uncomment the ones you want to load)



% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.






% *** CITATION PACKAGES ***
%

% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.
%
% Note that some packages require special options to format as the Computer
% Society requires. In particular, Computer Society  papers do not use
% compressed citation ranges as is done in typical IEEE papers
% (e.g., [1]-[4]). Instead, they list every citation separately in order
% (e.g., [1], [2], [3], [4]). To get the latter we need to load the cite
% package with the nocompress option which is supported by cite.sty v4.0
% and later.





% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex





% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath





% *** SPECIALIZED LIST PACKAGES ***
%\usepackage{acronym}
% acronym.sty was written by Tobias Oetiker. This package provides tools for
% managing documents with large numbers of acronyms. (You don't *have* to
% use this package - unless you have a lot of acronyms, you may feel that
% such package management of them is bit of an overkill.)
% Do note that the acronym environment (which lists acronyms) will have a
% problem when used under IEEEtran.cls because acronym.sty relies on the
% description list environment - which IEEEtran.cls has customized for
% producing IEEE style lists. A workaround is to declared the longest
% label width via the IEEEtran.cls \IEEEiedlistdecl global control:
%
% \renewcommand{\IEEEiedlistdecl}{\IEEEsetlabelwidth{SONET}}
% \begin{acronym}
%
% \end{acronym}
% \renewcommand{\IEEEiedlistdecl}{\relax}% remember to reset \IEEEiedlistdecl
%
% instead of using the acronym environment's optional argument.
% The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/acronym


%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array


%\usepackage{mdwmath}
%\usepackage{mdwtab}
% Also highly recommended is Mark Wooding's extremely powerful MDW tools,
% especially mdwmath.sty and mdwtab.sty which are used to format equations
% and tables, respectively. The MDWtools set is already installed on most
% LaTeX systems. The lastest version and documentation is available at:
% http://www.ctan.org/pkg/mdwtools


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.


%\usepackage{eqparbox}
% Also of notable interest is Scott Pakin's eqparbox package for creating
% (automatically sized) equal width boxes - aka "natural width parboxes".
% Available at:
% http://www.ctan.org/pkg/eqparbox




% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=footnotesize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a sans serif font rather
% than the serif font used in traditional IEEE formatting and thus the need
% to invoke different subfig.sty package options depending on whether
% compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig




% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix


%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
% endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% Axel Sommerfeldt. This package may be useful when used in conjunction with 
% IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% submissions have lists of figures/tables at the end of the paper and that
% figures/tables without any captions are placed on a page by themselves at
% the end of the document. If needed, the draftcls IEEEtran class option or
% \CLASSINPUTbaselinestretch interface can be used to increase the line
% spacing as well. Be sure and use the nomarkers option of endfloat to
% prevent endfloat from "marking" where the figures would have been placed
% in the text. The two hack lines of code above are a slight modification of
% that suggested by in the endfloat docs (section 8.4.1) to ensure that
% the full captions always appear in the list of figures/tables - even if
% the user used the short optional argument of \caption[]{}.
% IEEE papers do not typically make use of \caption[]'s optional argument,
% so this should not be an issue. A similar trick can be used to disable
% captions of packages such as subfig.sty that lack options to turn off
% the subcaptions:
% For subfig.sty:
% \let\MYorigsubfloat\subfloat
% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% However, the above trick will not work if both optional arguments of
% the \subfloat command are used. Furthermore, there needs to be a
% description of each subfigure *somewhere* and endfloat does not add
% subfigure captions to its list of figures. Thus, the best approach is to
% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% and instead reference/explain all the subfigures within the main caption.
% The latest version of endfloat.sty and its documentation can obtained at:
% http://www.ctan.org/pkg/endfloat
%
% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% later in the document, say, to conditionally put the References on a 
% page by themselves.





% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.

%\ifCLASSINFOpdf
%\usepackage[\MYhyperrefoptions,pdftex]{hyperref}
%\else
%\usepackage[\MYhyperrefoptions,breaklinks=true,dvips]{hyperref}
%\usepackage{breakurl}
%\fi
% One significant drawback of using hyperref under DVI output is that the
% LaTeX compiler cannot break URLs across lines or pages as can be done
% under pdfLaTeX's PDF output via the hyperref pdftex driver. This is
% probably the single most important capability distinction between the
% DVI and PDF output. Perhaps surprisingly, all the other PDF features
% (PDF bookmarks, thumbnails, etc.) can be preserved in
% .tex->.dvi->.ps->.pdf workflow if the respective packages/scripts are
% loaded/invoked with the correct driver options (dvips, etc.). 
% As most IEEE papers use URLs sparingly (mainly in the references), this
% may not be as big an issue as with other publications.
%
% That said, Vilar Camara Neto created his breakurl.sty package which
% permits hyperref to easily break URLs even in dvi mode.
% Note that breakurl, unlike most other packages, must be loaded
% AFTER hyperref. The latest version of breakurl and its documentation can
% be obtained at:
% http://www.ctan.org/pkg/breakurl
% breakurl.sty is not for use under pdflatex pdf mode.
%
% The advanced features offer by hyperref.sty are not required for IEEE
% submission, so users should weigh these features against the added
% complexity of use.
% The package options above demonstrate how to enable PDF bookmarks
% (a type of table of contents viewable in Acrobat Reader) as well as
% PDF document information (title, subject, author and keywords) that is
% viewable in Acrobat reader's Document_Properties menu. PDF document
% information is also used extensively to automate the cataloging of PDF
% documents. The above set of options ensures that hyperlinks will not be
% colored in the text and thus will not be visible in the printed page,
% but will be active on "mouse over". USING COLORS OR OTHER HIGHLIGHTING
% OF HYPERLINKS CAN RESULT IN DOCUMENT REJECTION BY THE IEEE, especially if
% these appear on the "printed" page. IF IN DOUBT, ASK THE RELEVANT
% SUBMISSION EDITOR. You may need to add the option hypertexnames=false if
% you used duplicate equation numbers, etc., but this should not be needed
% in normal IEEE work.
% The latest version of hyperref and its documentation can be obtained at:
% http://www.ctan.org/pkg/hyperref



% <-this % stops a space
%\IEEEcompsocitemizethanks{\IEEEcompsocthanksitem M. Shell was with the Department
%of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta,
%GA, 30332.\protect\\
% note need leading \protect in front of \\ to get a newline within \thanks as
% \\ is fragile and will error, could use \hfil\break instead.
%E-mail: see http://www.michaelshell.org/contact.html
%\IEEEcompsocthanksitem J. Doe and J. Doe are with Anonymous University.}% <-this % stops a space
%\thanks{Manuscript received April 19, 2005; revised August 26, 2015.}}

% note the % following the last \IEEEmembership and also \thanks - 
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
% 
% \author{....lastname \thanks{...} \thanks{...} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.

% Computer Society journal (but not conference!) papers do something unusual
% with the very first section heading (almost always called "Introduction").
% They place it ABOVE the main text! IEEEtran.cls does not automatically do
% this for you, but you can achieve this effect with the provided
% \IEEEraisesectionheading{} command. Note the need to keep any \label that
% is to refer to the section immediately after \section in the above as
% \IEEEraisesectionheading puts \section within a raised box.




% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps (small caps for compsoc).
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

% NOTE: PDF thumbnail features are not required in IEEE papers
%       and their use requires extra complexity and work.
%\ifCLASSINFOpdf
%  \usepackage[pdftex]{thumbpdf}
%\else
%  \usepackage[dvips]{thumbpdf}
%\fi
% thumbpdf.sty and its companion Perl utility were written by Heiko Oberdiek.
% It allows the user a way to produce PDF documents that contain fancy
% thumbnail images of each of the pages (which tools like acrobat reader can
% utilize). This is possible even when using dvi->ps->pdf workflow if the
% correct thumbpdf driver options are used. thumbpdf.sty incorporates the
% file containing the PDF thumbnail information (filename.tpm is used with
% dvips, filename.tpt is used with pdftex, where filename is the base name of
% your tex document) into the final ps or pdf output document. An external
% utility, the thumbpdf *Perl script* is needed to make these .tpm or .tpt
% thumbnail files from a .ps or .pdf version of the document (which obviously
% does not yet contain pdf thumbnails). Thus, one does a:
% 
% thumbpdf filename.pdf 
%
% to make a filename.tpt, and:
%
% thumbpdf --mode dvips filename.ps
%
% to make a filename.tpm which will then be loaded into the document by
% thumbpdf.sty the NEXT time the document is compiled (by pdflatex or
% latex->dvips->ps2pdf). Users must be careful to regenerate the .tpt and/or
% .tpm files if the main document changes and then to recompile the
% document to incorporate the revised thumbnails to ensure that thumbnails
% match the actual pages. It is easy to forget to do this!
% 
% Unix systems come with a Perl interpreter. However, MS Windows users
% will usually have to install a Perl interpreter so that the thumbpdf
% script can be run. The Ghostscript PS/PDF interpreter is also required.
% See the thumbpdf docs for details. The latest version and documentation
% can be obtained at.
% http://www.ctan.org/pkg/thumbpdf




% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol

% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.
% However, the Computer Society has been known to put floats at the bottom.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.



% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks









